Subset Sampling over Joins

Subset sampling (also known as Poisson sampling), where the decision to include any specific element in the sample is made independently of all others, is a fundamental primitive in data analytics, enabling efficient approximation by processing representative subsets rather than massive datasets. While sampling from explicit lists is well-understood, modern applications -- such as machine learning over relational data -- often require sampling from a set defined implicitly by a relational join. In this paper, we study the problem of \emph{subset sampling over joins}: drawing a random subset from the join results, where each join result is included independently with some probability. We address the general setting where the probability is derived from input tuple weights via decomposable functions (e.g., product, sum, min, max). Since the join size can be exponentially larger than the input, the naive approach of materializing all join results to perform subset sampling is computationally infeasible. We propose the first efficient algorithms for subset sampling over acyclic joins: (1) a \emph{static index} for generating multiple (independent) subset samples over joins; (2) a \emph{one-shot} algorithm for generating a single subset sample over joins; (3) a \emph{dynamic index} that can support tuple insertions, while maintaining a one-shot sample or generating multiple (independent) samples. Our techniques achieve near-optimal time and space complexity with respect to the input size and the expected sample size.

==> legacy.tex <==
\newpage

=======================PREVIOUS VERSION=====================







In addition, we will compute some additional statistics.
First, we construct the data structure described in Section~\ref{sec:static-index}, together with some additional statistics that we describe later. Recall that we will run Algorithm~\ref{alg:ss-rejected-batch} on the The main idea is that instead of invoking the \textsc{\bf FastRecursiveAccess} procedure separately for every pair $(\tau,\ell)$ found by Algorithm~\ref{alg:ss-rejected-batch}, we execute the \textsc{\bf FastRecursiveAccess} procedure for every node of $\T$ ``in parallel''. Notice that Algorithm~\ref{alg:fast-recursive} takes $O(\log \In)$ time because of the binary search in Step~1 and because of the computation of the smallest pair $(\ell_1,\ell_2)$ in Steps~4 and~5, since there are $O(\log \In)$ such pairs. 
In contrast, in the one-shot algorithm, for every node $R_i$ in $\T$, all smallest tuples $\bu$ and all smallest pairs $(\ell_1,\ell_2)$ for all pairs $(\tau,\ell)$ in $O(\In \cdot \log^2 \In + \beta^k \cdot \mu_\Psi)$ expected time. We then repeat the same procedure for every node of the tree, following a depth-first ordering. \xiao{any intuition here? or BFS is also fine?}
\stavros{Here I mean the following: In the previous section we assume that FastRecursiveAccess initially is called in the root. and then it follows a path: root->leftmostchild (line 9)->....-> again root with next child (line 10) and so on. Whatever was the ordering of that procedure in the previous section getting one subset sample, we follow exactly the same order here. Maybe the order is defined as (node,child) in Algorithm 5 instead of only node. But whatever that order was, we can folow the same order here.}


\paragraph{Algorithm}
The first step of our algorithm is the construction of the data structure from Section~\ref{sec:static-index}. We then compute some additional statistics. For every $\ell \in \llbracket L-1 \rrbracket$, every input relation $R_i$, and every $\bv \in R_i[\key(i)]$,  we construct a table $X_{i,\ell,\bv}$ of size $|R_i \ltimes \bv|$ such that for every $\bu \in R_i \ltimes \bv$, $X_{i,\ell,\bv}[\bu] = \sum_{\bu' \in R_i \ltimes \bv,\, \bu' \preceq \bu} W_{i,\bu'}(\ell)$. \xiao{how about $j$? In line 1, this is in terms of $W^j_{i,*}$}\stavros{Indeed, I forgot to add $j$ and the sum is over $W_{i,*}^j$}.
Next, for every $\ell \in \llbracket L-1 \rrbracket$, every input relation $R_i$, every $\bu \in R_i$, and every $R_j \in \C_i$, we construct a table $Y_{i,\ell,j,\bu}$ of size $O(\log_\beta \In)$ such that for every $(\ell_1,\ell_2)\in \Phi$ in lexicographically sorted order, $Y_{i,\ell,j,\bu}[(\ell_1,\ell_2)] = \sum_{(\ell_1',\ell_2') \preceq (\ell_1,\ell_2)\in\Phi} M_{j,\bu[\key(j)]}(\ell_1') \cdot W_{i,\bu}^{\next(j)}(\ell_2')$.

We execute \textsc{\bf FastRecursiveAccess} on every node of $\T$ “in parallel’’ among all triplets $(\tau,\ell,\bv)$ we need to satisfy. More formally, assume that the list of triplets for a node $R_i$ and a child $R_j\in\C_i$ is $P=\{(\tau^{(1)},\ell^{(1)},\bv^{(1)}),(\tau^{(2)},\ell^{(2)},\bv^{(2)}),\ldots\}$. Initially, $i=1$, $j=\emptyset$, and $P$ contains triplets of the form $(\tau^{(h)},\ell^{(h)},\emptyset)$\xiao{what is $h$? a random number?}\stavros{Yes, just an index. Sometime I use it instead of $\ell$.}, where $(\tau^{(h)},\ell^{(h)})$ are returned by Algorithm~\ref{alg:ss-rejected-batch}. We assume all scores $\ell^{(h)}<L$; otherwise, we compute the full join $\join(Q)$ and return all tuples in position $\tau^{(h)}$, exactly as in Section~\ref{sec:static-index}. This takes $O(1)$ expected time.

\xiao{Partition by which criteria?}\stavros{For every score $\ell$, we add in $P_\ell$ all triplets from $P$ with score $\ell$.}We partition the pairs $(\tau,\bv)$ in $P$ into $L$ groups: For each $h\in\llbracket L-1\rrbracket$ \xiao{what is $h$?}\stavros{similarly, as before, sometimes I used $h$ as $\ell$. For every score we define $P_\ell$.}, define $P_h=\{(\tau,\bv)\mid (\tau,h,\bv)\in P\}$.For each triplet $(\tau,\ell,\bv)\in P$, the goal is to compute the smallest tuple $\bu_{(\tau,\ell)}$ (step 1 of Algorithm~\ref{alg:fast-recursive}) \xiao{is it irrevalent to $\bv$?}\stavros{You are right that the computation of the smallest tuple in line 1 depends on $\bv$. So if it's more clear, we can use $\bu_{(\tau,\ell,\bv)}$. I skipped $\bv$ to simplify the notation because in any case all triplets  in $P$ have different pairs $(\tau,\ell)$. Also later, we use $\bu$ (in lines 5,6) and $\bv$ is irrelevant there.}. If $j\neq\emptyset$ (i.e., not the leftmost child), then $R_i\ltimes\bv$ contains exactly one tuple, so the smallest tuple is already known and the $\tau$-value in step 2 of Algorithm~\ref{alg:fast-recursive} does not change. Thus, we focus on the case $j=\emptyset$.

For each $P_\ell$, we sort all pairs $(\tau,\bv)$ by $\tau$ using radix sort~\cite{cormen2022introduction}. Let $(\tau_1,\bv_1)$ be the first pair. We traverse $X_{i,\ell,\bv_1}$ until we find the smallest $\bu_{(\tau_1,\ell)}$ with $X_{i,\ell,\bv_1}[\bu_{(\tau_1,\ell)}]\ge \tau_1$, and update $\tau_1$ according to step 2 of Algorithm~\ref{alg:fast-recursive}. For the next pair $(\tau_2,\bv_2)$, we continue the traversal of $X_{i,\ell,\bv_2}$ until we find the first $\bu_{(\tau_2,\ell)}$ satisfying $X_{i,\ell,\bv_2}[\bu_{(\tau_2,\ell)}]\ge \tau_2$, update $\tau_2$, and so on. If $\bv_h$ appears for the first time, we start at the beginning of $X_{i,\ell,\bv_h}$; otherwise, if $\bv_h=\bv_z$ for some $z<h$, we resume from the last visited position in $X_{i,\ell,\bv_z}$.
\xiao{there is something I didn't understand it. how to jump between different $\bv$ values?}
\stavros{Here we have many tables $X$. Each time we take the next sorted triplet $(\tau,\ell,\bv)$ in $P_\ell$ we first identify the table $X_{i,\ell,\bv}$ (also as you noted we will also have $j$) and then continue traversing the tuples from that specific table until we find the first tuple $\bu$ such that... Later, assume that we get another tuple $(\tau',\ell,\bv)$ in $P_\ell$ (same $\bv$ as in the previous case). Then we identify the same table $X_{i,\ell,\bv}$ and continue the traversal from $\bu$ we stopped earlier, we don't start the traversal fro mthe beginning of table $X_{i,\ell,\bv}$.}
Next, with updated $\tau$ values, we execute steps 4–6 of Algorithm~\ref{alg:fast-recursive}. For each $P_\ell$, we again sort all pairs by the updated $\tau$ values using radix sort.

Let $(\tau_1,\bv_1)$ be the first pair in $P_\ell$ and let $\bu'_1=\bu_{(\tau_1,\ell)}$ (recall that we computed $\bu_{(\tau_1, \ell)}$ earlier). We traverse $Y_{i,\ell,j,\bu'_1}$ until we find the first pair $(\ell_1^{(\tau_1,\ell)},\ell_2^{(\tau_1,\ell)})$ with $Y_{i,\ell,j,\bu'_1}[(\ell_1^{(\tau_1,\ell)},\ell_2^{(\tau_1,\ell)})]\ge \tau_1$, and update $\tau_1$ according to step 6 of Algorithm~\ref{alg:fast-recursive}. We then take the next pair $(\tau_2,\bv_2)$, let $\bu'_2=\bu_{(\tau_2,\ell)}$, and continue traversing $Y_{i,\ell,j,\bu'_2}$ until finding the corresponding smallest pair, updating $\tau_2$ accordingly. If $\bu'_h$ appears for the first time, we start the traversal from the beginning of $Y_{i,\ell,j,\bu'_h}$; otherwise, if $\bu'_h=\bu'_z$ for some $z<h$, we resume from the last visited element.

\newpage
=======================PREVIOUS VERSION=====================

We note that our data structure from Theorem~\ref{thm:best} directly yields an algorithm for the one-shot problem. Indeed, constructing the data structure and issuing one query produces a subset sample in $O(\In \cdot \log_\beta \In \cdot \log\log_\beta\In + \beta^k \cdot  \mu_\Psi\cdot \log \In)$ expected time, by combining the preprocessing time and query answering time. In this section, we show a specific algorithm for the one-shot version running in $O(\In \cdot \log^2\In + \beta^k \cdot \mu_\Psi)$ expected time, which is only required to return one subset sample. This result improves our previous result when $\mu_\Psi\gg \In$.

\smallskip
\noindent{\bf Algorithm.} We first keep all data statistics computed in the preprocessing phase as Section~\ref{sec:index-optimized}. We conceptually partition the join results into buckets. Recall that the high-level idea of answering one subset sampling is to use {\bf ss-rejected-batch} with instances $\{\langle \mathcal{B}_\ell, p \rangle: \ell \in \llbracket L-1\rrbracket\}$ with $p^+_{\ell} = \beta^{-\ell}$, and $\langle \bigsqcup_{\ell\ge L} \mathcal{B}_\ell, p \rangle$ with $p^+_{L} = \beta^{-L}$. Whenever a join result needs to be retrieved from  $\mathcal{B}_\ell$, if $\ell < L$, we use the \DA oracle to support the retrieval, and otherwise, we compute all the join results of $\bigsqcup_{\ell\ge L} \mathcal{B}_\ell$ to support the retrieval. In the first case, whenever the \DA oracle on bucket $\mathcal{B}_\ell$ with $\ell < L$ is invoked, it needs to pay $O(\log \In)$ time for each retrieval. Hence, to overcome this $O(\log \In)$ barrier in the query answering time, we need to compute additional statistics. Note that the second case is handled exactly the same as before. 

Careful inspection of Algorithm~\ref{alg:fast-recursive} reveals that the $O(\log \In)$ cost comes from the binary search in line \ref{locate-u} and the exhaustive search in line \ref{locate-score-pairs}. A natural idea is to precompute all these statistics. Consider an arbitrary relation $R_i \in Q$ with an arbitrary child node $R_j \in \C_i$. For every score $\ell \in \llbracket L-1 \rrbracket$, and every tuple $\bv \in R_i[\key(i)]$, we store an array $X_{i,j,\bv,\ell}$ of size $|R_i \ltimes \bv|$, where for every tuple $\bu \in R_i \ltimes \bv$, $$X_{i,j, \bv, \ell}(\bu) = \sum_{\bu' \in R_i \ltimes \bv,\, \bu' \preceq \bu} W^j_{i,\bu'}(\ell).$$ 
Next, for every score $\ell \in \llbracket L-1 \rrbracket$ and every tuple $\bu \in R_i$, we store an array $Y_{i,j,\ell,\bu}$ of size at most $L$, where for every pair $(\ell_1,\ell_2)\in \llbracket \ell\rrbracket$ with $\ell_1 + \ell_2 = \ell - \phi(\bu)$,  lexicographically sorted order, $$Y_{i,j,\bu, \ell}(\ell_1,\ell_2) = \sum_{(\ell_1,\ell_2)\in \llbracket \ell \rrbracket: (\ell_1',\ell_2') \preceq (\ell_1,\ell_2), \ell_1 + \ell_2 = \ell - \phi(\bu)} M_{j,\bu[\key(j)]}(\ell_1') \cdot W_{i,\bu}^{\textrm{next}(j)}(\ell_2').$$ 

Each invocation of Algorithm~\ref{alg:fast-recursive} is identified by a quintuples $(i,j,\bv,\ell,\tau)$ as its input. 
The high-level idea is to maintain the list of quintuples $(i,j,\bv,\ell,\tau)$ on which we will invoke Algorithm~\ref{alg:fast-recursive}, and run multiple invocations of Algorithm~\ref{alg:fast-recursive} together by merging some certain operations. A quintuple $(i',j',*,*,*)$ is dominated by another one $(i,j,*,*,*)$, if $R_i$ is an ancestor of $R_{i'}$ in $\T$, or if $R_j \prec R_{j'}$ when $i=i'$. In other words, we consider handling the quintuples in a lexicographically increasing order of $(i,j)$. Moreover, we will group these quintuples by $(i,j,\bv,\ell)$, where quintuples inside each group only have different $\tau$-values sorted by $\tau$ in an increasing order.

Initially, for each sample request issued by {\bf ss-rejected-batch}, in a form of $(\ell, \tau)$ with $\ell \in  \llbracket L -1\rrbracket$, indicating that the $\tau$-th join result in the bucket $\mathcal{B}_\ell$ is sampled, we add a quintuple $(r,\emptyset, \emptyset, \ell, \tau)$ for the root node $R_r$ to $\calP$. So far, all quintuples in $\calP$ have the same value of $i=r$, $j=\emptyset$ and $\bv = \emptyset$. We will put these quintuples into groups by $(r,\emptyset,\emptyset,\ell)$, where again each group only has different $\tau$-values sorted by $\tau$ in an increasing order. Note that this is done by applying radix sorting algorithm \cite{} to all quintuples in $\calP$ by $\tau$. Then, we go through each quintuple in the sorted $\calP$ and assign it to the specific group indexed by $(r,\emptyset,\emptyset,\ell)$. 

First, we execute line \ref{locate-u} for all these invocations of Algorithm \ref{alg:fast-recursive}. Recall that it computes the smallest tuple $\bu$ in $R_i \ltimes \bv$ such that $\sum_{\bu' \in R_i \ltimes \bv: \bu'\preceq\bu} W^j_{i,\bu'}(\ell) \ge \tau$. Hence, we will find the specific tuple $\bu$ for each quintuple $(r,\emptyset, \emptyset, \ell, \tau) \in \calP$ by an increasing order of $\tau$, which can be done by a linear scan of the auxiliary array $X_{r, \emptyset, \emptyset, \ell}$. Meanwhile, for each quintuple $(r,\emptyset, \emptyset, \ell,\tau)$, we need to update its rank $\tau$ according to line \ref{correct-index-u} and update the $\bv$-value to it with its own $\bu$, which results in a new quintuple $(r,\emptyset, \bu, \ell, \tau)$. 
After this step, we put these quintuple into groups by $(i,j,\bu,\ell)$, where again each group only have different $\tau$-values sorted by $\tau$ in an increasing order. Note that this is done by applying radix sorting algorithm \cite{} \todo{} to all quintuples in $\calP$ by $\tau$. Then, we go through each quintuple in the sorted $\calP$ and assign it into the specific group indexed by $(i,j,\bu,\ell)$. 

\renewcommand{\P}{\mathcal{P}}
\begin{algorithm}[t]   \caption{$\textsc{MergeRecursiveAccess}(\{(\ell,\tau)\} \todo{...})$}
    \label{alg:one-shot}
    \todo{to be moved to appendix.}
    \For{each $R_i \in Q$}{
    \For{each $R_j \in \C_i$}{
        $\calP_{i,j} \gets \emptyset$\;
    }
    }
    \For{each $(\ell,\tau)$ issued by {\bf ss-rejected-batch}}{
    $\calP_{r,\emptyset} \gets \calP_{r,\emptyset} \cup \{(r,\emptyset, \emptyset, \ell, \tau)\}$\;
    }
    \For{each $R_i \in Q$ in pre-order of $\T$}{
    \For{each $R_j \in \{\emptyset\} \circ \C_i$ in pre-order of $\T$}{
        Sort quintuples in $\calP_{i,j}$ by $\tau$ using radix sort algorithm\;
        Group $\calP_{i,j}$ further by $(i,j,\bv,\ell)$, where quintuples in each group $\calP_{i,j,\bv,\ell}$ are increasingly ordered by $\tau$\;
        \For{each $(i,j,\bv,\ell)$}{
            $\bu \gets$ the first tuple in $ X_{i,j,\bv,\ell}$\;
            \While{some quintuple in $\calP_{i,j,\bv,\ell}$ is not updated}{
             $(i,j,\bv,\ell,\tau) \gets$ the first non-visited quintuple in $\calP_{i,j,\bv,\ell}$\;
             \lWhile{$X_{i,j,\bv,\ell}(\bu) < \tau$}{
                $\bu \gets$ the next tuple in $ X_{i,j,\bv,\ell}$}
                Update $(i,j,\bv,\ell,\tau)$ to $(i,j,\bu,\ell,\tau - X_{i,j,\bv,\ell}(\textsf{prev}(\bu)))$\;
                \lIf{$R_i$ is a leaf node}{\todo{in the base case, how to return tuples and concatenate them into join results}}
                }
            }
        Sort quintuples in $\calP_{i,j}$ by $\tau$ using radix sort algorithm\;
        Group $\calP_{i,j}$ further by $(i,j,\bu,\ell)$, where quintuples in each group $\calP_{i,j,\bu,\ell}$ are increasingly ordered by $\tau$\;
        \For{each $(i,j,\bu,\ell)$}{
            $(\ell_1,\ell_2) \gets$ the first pair in $ Y_{i,j,\bu,\ell}$\;
            \While{some quintuple in $\calP_{i,j,\bu,\ell}$ is not visited}{
             $(i,j,\bu,\ell,\tau) \gets$ the first non-visited quintuple in $\calP_{i,j,\bu,\ell}$\;
             \lWhile{$Y_{i,j,\bu,\ell}(\ell_1,\ell_2) < \tau$}{
                $(\ell_1,\ell_2) \gets$ the next pair in $ Y_{i,j,\bu,\ell}$
            }
            Compute $\tau_1, \tau_2$ based on $\ell_1, \ell_2$ according to lines \ref{left-index}-\ref{right-index} of Algorithm~\ref{alg:fast-recursive}\;
            $\mathcal{P}_{i,j} \gets \mathcal{P}_{i,j} - \{(i,j,\bu,\ell,\tau)\}$\; 
             $\mathcal{P}_{j,\emptyset} \gets \mathcal{P} \cup \{(j,\emptyset, \bu,\ell_1,\tau_1)\}$\; 
            $\mathcal{P}_{i,\textrm{next}(j)} \gets \mathcal{P} \cup \{(i,\textrm{next}(j),\bu,\ell_2,\tau_2)\}$\; 
             
            }
        }
    }
}
\end{algorithm}






Next, we execute line \ref{locate-score-pairs} for all these invocations of Algorithm \ref{alg:fast-recursive} together.  Recall that it computes smallest pair $(\ell_1, \ell_2)$ such that 
$$
\displaystyle{\sum_{(\ell'_1,\ell'_2) \in \llbracket \ell \rrbracket: (\ell'_1,\ell'_2) \preceq (\ell_1, \ell_2), \ell'_1+\ell'_2 =\ell - \phi(\bu)} M_{j, \bu[\key(j)]}(\ell_1') \cdot W^{\textsf{next}(j)}_{i, \bu}(\ell_2') \ge \tau}.
$$ 
This time, we will find the specific pair $(\ell_1,\ell_2)$ for each quintuple $(r,\emptyset, \bu,\ell, \tau) \in \calP$, which can be done by a linear scan of the auxiliary array $Y_{r, \emptyset, \bu, \ell}$. Meanwhile, for each quintuple $(r,\emptyset, \bu,\ell, \tau)$, we need to update its rank $\tau$ according to line \ref{correct-index-score-pairs} and compute new indices $\tau_1,\tau_2$ according to lines \ref{left-index}-\ref{right-index}. We then remove $(r,\emptyset, \bu,\ell, \tau)$ from $\calP$ and add two new quintuples $(j^\circ,\emptyset, \bu, \ell_1 ,\tau_1)$ and $(r,j^\circ,\bu, \ell_1,\tau_2)$ to $\calP$, where $j^\circ$ is the first child node of root node $R_r$.

Now, we have quintuples $i = j^\circ$ are dominated by those with $i = r$. We will recursively apply this procedure on quintuples are not dominated.  \todo{in the base case, how to return tuples and concatenate them into join results}

\smallskip
\noindent{\bf Analysis.}
The correctness follows directly from Theorem~\ref{thm:best}. We are exactly simulating the execution of all invocations of Algorithm~\ref{alg:fast-recursive}. Next, we focus on the running time of the algorithm.
The data statistics inheriting from Theorem~\ref{thm:best} can be computed in $O(\In\log_\beta(\In)\log\log_\beta(\In))$ time. All $X$-arrays can be computed in $O(\In\log_\beta\In)$ time. All $Y$-arrays can be computed in $O(\In\log_\beta^2\In)$ time, since there are $O(\In\log_\beta\In)$ arrays and each array can be computed in $O(\log_\beta\In)$ time.



\todo{below: to be formalized and adapted to the definition on quintuples.}

As $\tau \in \llbracket N^{\rho^*}\rrbracket$, the radix sort algorithms runs in $O(\In+|\calP|)$ time. 
Overall, all groups $P_\ell$ are sorted in $\sum_{\ell\in \llbracket L-1\rrbracket}O(\In+|P_\ell|)=O(\In\log_\beta \In+\beta^k\mu_\Psi)$ expected time.

To compute all $\bu_{(\tau,\ell)}$, we iterate over all triplets in $P$ and traverse all $X$ tables once in the worst case. Since for every $\bu \in R_i$ there is a unique $\bv$ with $\bu \in R_i\ltimes\bv$, we have $\sum_{i,\ell,\bv}|X_{i,\ell,\bv}|=O(\In\log_\beta\In)$. Thus the cost is $O(\In\log_\beta\In + \beta^k\mu_\Psi)$ expected time.
Similarly, computing all pairs $(\ell_1^{(\tau,\ell)},\ell_2^{(\tau,\ell)})$ requires a single pass over all triplets in $P$ and all $Y$ tables. Since there are $O(\In\log_\beta\In)$ tables $Y$ of size $O(\log_\beta\In)$, the total cost is $O(\In\log_\beta^2\In + \beta^k\mu_\Psi)$ expected time. Overall, the running time of the one-shot algorithm is $O(\In\log_\beta^2\In + \beta^k\mu_\Psi)$ expected time.



Overall, we conclude with the next theorem.
\newpage


In
addition, we compute the following statistics for each relation $R_i \in Q$. For each tuple $\bv \in R_i[\key(i)]$, we recall an ordering on tuples in $R_i \ltimes \bv=\{\bv_1,\ldots,\bv_{|R_i \ltimes \bv|}\}$, which inherits the ordering of tuples in $R_i$. For all $j \in [|R_i \ltimes \bv|]$, we further define:
\begin{equation}
    \label{eq:M}
    M^j_{i,\bv}(\ell) = \sum^{j}_{z = 1} W_{i,\bv_z}(\ell).
\end{equation}


By this definition, we have $M^{|R_i \ltimes v|}_{i,\bv}(\ell) = M_{i,\bv}(\ell)$.
%In other words, the values $M^j_{i,\bv}(\ell)$ store a prefix sum of the values $W_{i,\bv_z}(\ell)$.

Moreover, for all $R_i \in Q$, let $\{ R_{i_1}, \ldots, R_{i_{|C_i|}} \} = C_i$, denote an ordering of the children relations of $R_i$. For all relations $R_i \in Q$, and for all $j \in [|C_i|]$, we define $\T_i^j$ to be the subtree of relation $R_i$, except for the first $j$ children of $R_i$. Formally, for $j \in [|C_i|]$, we define $\T_i^j = \T_i - \cup_{z = 1}^j\T_{i_j}$ and we define $\T^{0}_{i} = \T_i$. For each tuple $\bu \in R_i$ and each index $j \in [|C_i|]$, we compute $L+1$ counters $W^j_{i,\bu}(0), W^j_{i,\bu}(1), \ldots, W^j_{i,\bu}(L)$: for $\ell \in \llbracket L \rrbracket$ and $j \in [|C_i|] \cup \{0\}$, $W^j_{i,\bu}(\ell)$ stores the number of join results produced by relations in the subtree $\T^j_i$ that is also participated by $\bu$, with score $\ell$, i.e., 

    $$W^j_{i,\bu}(\ell) = \left|\left\{\bm{t} \in (\Join_{R_z \in \T^j_i} R_z)\ltimes \bu: \ \min\left\{L, \ \ \sum_{R_z \in \T^j_i} \phi(\bm{t}[\schema(R_z)])\right\} = \ell\right\}\right|.$$
If $j=|C_i|$, we set $W_{i,\bu}^j(\ell)=1$. \aryan{Why do we have this?}
Notice that for both $M$ and $W$, we also have a definition without the superscript $j$. By our new definition, the superscript $j$ defines a partial sum over the values, which we will need later to be able to efficiently access the desired tuples.

Having these statistics, we define a procedure \textsc{\bf FastRecursiveAccess}$(\T, i, j, \bu, \ell, \tau)$, that returns the tuple number $\tau$, in the join of the relations in the subtree $\T_i^{j - 1}$, with score $\ell$, that $u\in R_i$ participates in. This is based on an arbitrary but fixed ordering of the tuples in the result of the join of $\T_i^j$.

% \newpage
% \mytab{
%     \> {\bf RecursiveAccess}$(T, i, j, \bu, \ell, \tau)$ \\ 

%     \> $/*$ Subtracting the score of the tuple $u$ itself from the total score $\ell$ $*/$\\
%     \> 1.\> $\ell \gets \ell - \phi(\bu)$; \\[2pt]

%     \> $/*$ Recall $C_i = \{R_{i_1}, R_{i_2}, \ldots\}$ are the children relations of $R_i$. \\ 
%     \>\ \ \ We are only considering the children $\{R_{i_j}, R_{i_{j+1}}, \ldots\}$ by definition of this function. $*/$\\
%     \> 2.\> $\ell_j \gets 0$; \quad $/*$ How much score we spend in child $R_{i_j}$ $*/$ \\[4pt]

%     \> 3.\> $v \gets \bu[\key(i_j)]$; \\[6pt]

%     \> $/*$ 
%         We initialize $S$ by the number of tuples we can create if we spend $0$ in the subtree of $R_{i_j}$  
%         and $\ell$ in the remaining children 
%        $*/$\\

       
%     \> 4.\> $S \gets M_{i_j,v}[0] \cdot W_{i,u}^{j}(\ell)$; \\[6pt]

%     \> 5.\> $\tau' \gets \tau$; \\[4pt]

%     \> $/*$ In the while loop, we find the value of $\ell_j$ $*/$\\
%     \> 6.\> {\bf while} $S < \tau$ {\bf do} \\
%     \> 7.\>\> $\tau' \gets \tau' - M_{i_j,v}[\ell_j] \cdot W_{i,u}^{j}[\ell - \ell_j]$; \\
%     \> 8.\>\> $\ell_j \gets \ell_j + 1$; \\
%     \> 9.\>\> $S \gets S + M_{i_j,v}[\ell_j] \cdot W_{i,u}^{j}[\ell - \ell_j]$; \\[6pt]

%     \> $/*$ After finding $\ell_j$, how much score we spend on children $\{R_{i_{j+1}}, \ldots\}$ $*/$\\
%     \> 10.\> $\ell_{\text{right}} \gets \ell - \ell_j$; \\[8pt]

%     \> $/*$ 
%          Recall $R_{i_j} \ltimes v = \{v_1, \ldots, v_{|R_{i_j} \ltimes v|}\}$ is the ordered list of tuples  
%          in $R_{i_j}$ joinable with $u$.  
%          We want to find the tuple $v_h$ to recurse on. 
%        $*/$\\[2pt]
%     \> $/*$ 
%          $h =$ xsmallest index such that  
%          $M^{h}_{i_j, v}[\ell_j] \cdot W_{i,u}^{j}[\ell_{\text{right}}] \ge \tau'$.  
%          (Found by binary search.)
%        $*/$\\
%     \> 11.\> $h \gets$ smallest index $h$ such that \\ 
%     \>\>\>\> $M^{h}_{i_j, v}[\ell_j] \cdot W_{i,u}^{j}[\ell_{\text{right}}] \ge \tau'$; \\[8pt]

%     \> $/*$ Remove contributions of all blocks before $h$ $*/$\\
%     \> 12.\> $\tau' \gets \tau' - M^{h - 1}_{i_j, v}[\ell_j] \cdot W_{i,u}^{j}[\ell_{\text{right}}]$; \\[8pt]

%     \> $/*$ 
%          $\tau_j =$ the index of the tuple coming from the subtree of $R_{i_j}$  
%          that joins with $v_h$ 
%        $*/$\\
%     \> 13.\> $\tau_j \gets \left\lceil \dfrac{\tau'}{W_{i,u}^{j}[\ell_{\text{right}}]} \right\rceil$; \\[8pt]

%     \> $/*$ 
%          $\tau_{\text{right}} =$ the index of the tuple chosen from the right children  
%          that joins with $u$ 
%        $*/$\\
%     \> 14.\> $\tau_{\text{right}} \gets (\tau' \bmod W_{i,u}^{j}[\ell_{\text{right}}]) + 1$; \\[12pt]

%     \> 15.\> {\bf return} $u \Join$ {\bf RecursiveAccess}$(T, i_j, 0, v_h, \ell_j, \tau_j) \Join$ {\bf RecursiveAccess}$(T, i, j+1, \bu, \ell_{\text{right}}, \tau_{\text{right}})$; \\
% }
\begin{algorithm}[t]
    \caption{\textsc{\bf FastRecursiveAccess}$(\T, i, j, \bu, \ell, \tau)$}
    \label{alg:recursive-access-efficient}
    \lIf{$R_i$ is a leaf node}{\Return $u$}
    \tcp{Subtracting the score of the tuple $u$ itself from the total score $\ell$}
    $\ell' \gets \ell - \phi(\bu)$\;
    \tcp{Recall $C_i = \{R_{i_1}, R_{i_2}, \ldots\}$ are children of $R_i$. We consider children $\{R_{i_j}, \ldots\}$.}
    $\ell_j \gets 0$ \tcp*[r]{How much score we spend in child $R_{i_j}$}
    $v \gets \bu[\key(i_j)]$\;
    \tcp{Initialize $S$ by tuples created if we spend $0$ in $R_{i_j}$ subtree and $\ell'$ in remaining children}
    $S \gets M_{i_j,v}[0] \cdot W_{i,u}^{j}[\ell']$\;
    $\tau' \gets \tau$\;
    \tcp{In the while loop, we find the value of $\ell_j$}
    \While{$S < \tau$}{
        $\tau' \gets \tau' - M_{i_j,v}[\ell_j] \cdot W_{i,u}^{j}[\ell' - \ell_j]$\;
        $\ell_j \gets \ell_j + 1$\;
        $S \gets S + M_{i_j,v}[\ell_j] \cdot W_{i,u}^{j}[\ell' - \ell_j]$\;
    }
    \tcp{After finding $\ell_j$, how much score we spend on children $\{R_{i_{j+1}}, \ldots\}$}
    $\ell_{\text{right}} \gets \ell' - \ell_j$\;
    \tcp{Find tuple $v_h$ to recurse on via binary search on $R_{i_j} \ltimes v$}
    $h \gets$ smallest index $h$ such that $M^{h}_{i_j, v}[\ell_j] \cdot W_{i,u}^{j}[\ell_{\text{right}}] \ge \tau'$\;
    \tcp{Remove contributions of all blocks before $h$}
    $\tau' \gets \tau' - M^{h - 1}_{i_j, v}[\ell_j] \cdot W_{i,u}^{j}[\ell_{\text{right}}]$\;
    \tcp{$\tau_j =$ index of tuple from subtree of $R_{i_j}$ joining with $v_h$}
    $\tau_j \gets \left\lceil \dfrac{\tau'}{W_{i,u}^{j}[\ell_{\text{right}}]} \right\rceil$\;
    \tcp{$\tau_{\text{right}} =$ index of tuple from right children joining with $u$}
    $\tau_{\text{right}} \gets ((\tau'-1) \bmod W_{i,u}^{j}[\ell_{\text{right}}]) + 1$\;
    \Return $u \Join$ \textsc{\bf FastRecursiveAccess}$(\T, i_j, 0, v_h, \ell_j, \tau_j) \Join$ \textsc{\bf FastRecursiveAccess}$(\T, i, j+1, \bu, \ell_{\text{right}}, \tau_{\text{right}})$\;
\end{algorithm}
%\todo{There are some bases cases missing in the code above.}
Without loss of generality, let $R_1$ be the root of $\T$. Recall that our goal is for any bucket $\mathcal{B}_\ell$, given any integer $\tau \in [|\mathcal{B}_\ell|]$, to return the $\tau$-th tuple in bucket $B_\ell$. 
The \textsc{\bf FastRecursiveAccess} procedure has as an input parameter a tuple $u \in R_1$ that is used from the first relation. To find such a tuple $u \in R_1$, we execute a binary search to identify the smallest tuple (with respect to our arbitrary ordering of tuples in $R_1$), such that $\sum_{u' \in R_1, \bu' \leq u}W_{1,u'}[l] \geq \tau$. This is straightforward to do by maintaining a prefix sum over $W_{1, \bu}[l]$, for the varying value of $u$ and each fixed $l$.
We then call {\bf RecursiveAccess-E$(\T, 1, 1, \bu, l, \tau - \sum_{u' \in R_1, \bu' < u}W_{1,u'}[l])$} to get our desired tuple.

\paragraph{Main idea}

\paragraph{Description of the \textsc{\bf FastRecursiveAccess} procedure}

\paragraph{Correctness and analysis}
\begin{lemma}
\label{lem:bestCorr}
    The \textsc{\bf FastRecursiveAccess} procedure is correct.
\end{lemma}
\begin{proof}
    
\end{proof}



\begin{lemma}
\label{lem:bestRun-legacy}
The \textsc{\bf FastRecursiveAccess} procedure runs in $O(\log \In)$ time.  
\end{lemma}
\begin{proof}
Let fix a node $R_i$ and a parameter $j$.
All steps up to line 7 run directly in $O(1)$ time.
The While loop in lines 8--11 is executed at most $\ell'=O(\log_\beta(\In))$ times. 
By definition, the number of join results with score $\ell'$ in $\T_i^j$ that are joined with $u$ is $\sum_{\lambda\in \llbracket \ell'\rrbracket}M_{i_j,v}[\lambda]\cdot W_{i,u}^j[\lambda-\ell_j]$.
If $S<\tau$ when $\ell_j=\ell'$, then $\tau>\sum_{\lambda\in \llbracket \ell'\rrbracket}M_{i_j,v}[\lambda]\cdot W_{i,u}^j[\lambda-\ell_j]$, which is a contradiction because of the correctness proof, i.e., for every call of \textsc{\bf FastRecursiveAccess}$(\T, i, j, \bu, \ell, \tau)$ the value of $\tau$ is at most the number of join results with score $\ell'$ in $\T_i^j$ that are joined with $u$.
In fact, it is easy to observe a stronger property: We always set $\ell'=\ell-\phi(\bu)$, so the total number of the while loop in lines 8--11 over all the nodes of $\T$ is still bounded by $O(\log_\beta \In)$.


    Next, the algorithm runs a binary search on the tuples of $R_{i_j}\ltimes v$. We have $|R_{i_j}\ltimes v|=O(\In)$ so this step takes $O(\log \In)$ time. A;l remaining steps of the procedure run straightforwardly in $O(1)$ time.
\end{proof}



\subsection{Preprocessing}
In this section, we discuss how to compute the needed statistics for the direct access algorithm efficiently. For each relation $R_i \in Q$, each tuple $u \in R_i$, each index $j \in \llbracket|C_i|\rrbracket$, and each score $\ell \in \llbracket L \rrbracket$, we compute $W^j_{i,u}(\ell)$ as follows. If $R_i$ is a leaf node in $\T$, then $C_i = \emptyset$, and we have $W^0_{i, \bu}[\phi(\bu)] = W_{i, \bu}[\phi(\bu)] = 1$ and for all $\ell \neq \phi(\bu)$, we have $W^0_{i, \bu}(\ell) = W_{i, \bu}(\ell) = 0$. If $R_i$ is not a leaf, then we have $W^{j}_{i, \bu}(\ell) = \sum^{\ell}_{z = 0}M_{i_j, \bu[\key(i_j)]}[z] \cdot W^{j + 1}_{i, \bu}[\ell - z]$, for all $j \in 
%\{0, \cdots, |C_i| - 1\}
\llbracket|C_i| - 1\rrbracket
$. We set $W^{|C_i|}_{i, \bu}[0] = 1$, and $W^{|C_i|}_{i, \bu}(\ell) = 0$, for all $\ell > 0$. Next, we describe how to calculate the values of $M$. We first set $M^0_{i, v}[l] = 0$, for all $\ell \in \llbracket L \rrbracket$. Then, we have $M^{j}_{i, v}[l] = M^{j - 1}_{i, v}(\ell) + W_{i, v_j}(\ell)$, for all $j > 0$ and for all $\ell \in \llbracket L \rrbracket$. 

\aryan{I think it is cleaner to remove the definition of $W$ without the superscript and use the notation $W^0$ instead.} 

Given the join tree $\T$ of the query $Q$, we start from the leaf nodes. When processing the node $R_i$, we first calculate $W$, then, having $W$, we calculate the values of $M$. We define the {\bf Preprocess} procedure as follows. At the beginning of our algorithm, we just call {\bf Preprocess$(\T, i)$}, to compute all the values of  $W$ and $M$. 

\noindent \textbf{Complexity Analysis.} The running time of the \textbf{Preprocess} procedure is primarily dominated by the computation of the intermediate weight tables. In its direct implementation described, the algorithm has a time complexity of $O(\In \cdot L^2)$.

To see this, observe that the base cases and the initialization of leaf nodes execute in time linear in $L$ for each tuple. Hence, the computational bottleneck arises during the recursive step, specifically within the nested loops used to combine results from children (Lines 11--16). The update rule is defined as:
\[
    W^j_{i,u}(\ell) = \sum_{z=0}^{\ell} M_{i_j, \bu[\key(i_j)]}[z] \cdot W^{j+1}_{i,u}[\ell - z]
\]
This expression represents the \textit{discrete convolution} of the score distribution array $M$ (associated with the current child) and the weight array $W$ (associated with the previously processed children). In the naive iterative approach, computing this sum for a single value $\ell$ requires $O(\ell)$ operations. Iterating over all $\ell \in 
%\{0, \dots, L\}
\llbracket L\rrbracket
$ results in $O(L^2)$ operations per tuple. When aggregated over the total input size $\In$, the overall complexity is $O(\In \cdot L^2)$.

\noindent \textbf{Optimization via FFT.} The running time can be improved by recognizing the convolution structure. Since $M$ and $W$ are arrays of length $L+1$, their convolution can be computed efficiently using the Fast Fourier Transform (FFT). By transforming the arrays into the frequency domain, performing point-wise multiplication, and applying the inverse FFT, the convolution cost is reduced from $O(L^2)$ to $O(L \log L)$. Applying this technique reduces the total running time of the algorithm to $O(\In \cdot L \log L)$.

\begin{theorem}
\label{thm:bestold}
Given an acyclic join instance $Q$ and a set of associated weight functions $\{\fp_j\}_{R_j \in Q}$, there exists a data structure $\D$ of size $O(\In\cdot \log_\beta\In)$ that can be built in  $O(\In\cdot \log_{\beta} \In\cdot \log_2(\log_\beta \In))$ time, such that each subset sampling query can be answered in $O(1+\beta^k\mu_\Psi\log \In)$ expected time.
%, which is optimal in the expected sense if $\beta=O(1)$.
\end{theorem}
\begin{proof}
The space and the preprocessing time follow directly from our analysis above.

For the query procedure, we execute Algorithm~\ref{alg:ss-rejected-batch} using the \textsc{\bf FastRecursiveAccess} procedure for the direct access procedure. Notice that from the preprocessing, we have $L=O(\log_\beta\In)$ buckets and for each $\ell \in \llbracket L \rrbracket$, we know its size.
%Let $\ell$ be the bucket (score) selected by Algorithm~\ref{alg:ss-rejected-batch} in one iteration and let $\tau$ be the value returned by the Geometric (or Truncated Geometric) distribution.
If the bucket $B_\ell$ for $\ell=L=2k\log \In$ is selected by Algorithm~\ref{alg:ss-rejected-batch}, then we evaluate the full join $\join(Q)$ and and for every $\tau$ selected by the Geometric (or Truncated Geometric distribution) we return its $\tau$-th tuple (according to an arbitrary but fixed ordering of the tuples). 
If any other bucket $B_\ell$ is selected, then for each $\tau$ we call the \textsc{\bf FastRecursiveAccess} procedure. 

The correctness of the query procedure of the follows directly from Algorithm~\ref{alg:ss-rejected-batch} and Lemma~\ref{lem:bestCorr}.

The probability that at least one tuple from the bucket $L$ is selected is at most $\frac{1}{\In^k}$. Evaluating the full join $\join(Q)$ takes $O(\In^k)$ time, so in expectation this step runs in $O(1)$ time.
   In any other case, from Lemma~\ref{lm:nss} and Lemma~\ref{lem:bestRun}, the overall expected running time of the query procedure is $O(1+\beta^k\mu_\Psi\log \In)$.
\end{proof}
